TactileEval: A Step Towards Automated Fine-Grained Evaluation and Editing of Tactile Graphics

Tactile graphics require careful expert validation before reaching blind and visually impaired (BVI) learners, yet existing datasets provide only coarse holistic quality ratings that offer no actionable repair signal. We present TactileEval, a three-stage pipeline that takes a first step toward automating this process. Drawing on expert free-text comments from the TactileNet dataset, we establish a five-category quality taxonomy; encompassing view angle, part completeness, background clutter, texture separation, and line quality aligned with BANA standards. We subsequently gathered 14,095 structured annotations via Amazon Mechanical Turk, spanning 66 object classes organized into six distinct families. A reproducible ViT-L/14 feature probe trained on this data achieves 85.70% overall test accuracy across 30 different tasks, with consistent difficulty ordering suggesting the taxonomy suggesting the taxonomy captures meaningful perceptual structure. Building on these evaluations, we present a ViT-guided automated editing pipeline that routes classifier scores through family-specific prompt templates to produce targeted corrections via gpt-image-1 image editing. Code, data, and models are available at https://TactileEval.github.io/

==> pipeline.tex <==
\begin{figure*}[t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    font=\small,
    data/.style  ={rectangle, rounded corners=5pt, draw=blue!60!black,
                   fill=blue!10, text centered, minimum height=1.1cm,
                   minimum width=2.0cm, text width=1.9cm, line width=0.8pt},
    model/.style ={rectangle, rounded corners=5pt, draw=orange!70!black,
                   fill=orange!12, text centered, minimum height=1.1cm,
                   minimum width=2.0cm, text width=1.9cm, line width=0.8pt},
    output/.style={rectangle, rounded corners=5pt, draw=green!50!black,
                   fill=green!10, text centered, minimum height=1.1cm,
                   minimum width=2.0cm, text width=1.9cm, line width=0.8pt},
    phase/.style ={font=\footnotesize\bfseries, text=gray!60!black},
    arr/.style   ={->, very thick, >=stealth},
]

%% ── Row 1: Data pipeline (all on y=0) ──────────────────────────────
\node[data] (A) at (0,0)   {\textbf{Expert}\\Comments};
\node[data] (B) at (2.8,0) {\textbf{Taxonomy}\\
                             \footnotesize F1QB, F1QP\\F1QT, F1QL, F1QV};
\node[data] (C) at (5.6,0) {\textbf{AMT}\\
                             \footnotesize 231 HITs\\per family};
\node[data] (D) at (8.4,0) {\textbf{JSONL Splits}\\
                             \footnotesize 5{,}266 / 557 / 578};

%% ── Evaluators: E1 above, E2 below ─────────────────────────────────
\node[model] (E1) at (11.4, 1.1)  {\textbf{GPT-4o}\\
                                    \footnotesize Pilot (3.2\%)\\
                                    \footnotesize 76.04\% acc.};
\node[model] (E2) at (11.4,-1.1)  {\textbf{CLIP Probe}\\
                                    \footnotesize Full dataset\\
                                    \footnotesize 87.38\% acc.};

%% ── Output: F and G back on y=0 ────────────────────────────────────
\node[output] (F) at (14.4, 0)    {\textbf{Diagnosis}\\
                                    \footnotesize + Edit Plan\\
                                    \footnotesize (few-shot)};
\node[output] (G) at (17.2, 0)    {\textbf{Corrected}\\
                                    \footnotesize Tactile Render\\
                                    \footnotesize \texttt{gpt-image-1}};

%% ── Section labels ──────────────────────────────────────────────────
\node[phase] at (0,    0.95) {\S III};
\node[phase] at (2.8,  0.95) {\S III};
\node[phase] at (5.6,  0.95) {\S IV};
\node[phase] at (8.4,  0.95) {\S V};
\node[phase] at (11.4, 2.05) {\S V-B};
\node[phase] at (11.4,-2.05) {\S V-C};
\node[phase] at (14.4, 0.95) {\S VI};
\node[phase] at (17.2, 0.95) {\S VI};

%% ── Arrows ──────────────────────────────────────────────────────────
\draw[arr, blue!60!black]   (A)  -- (B);
\draw[arr, blue!60!black]   (B)  -- (C);
\draw[arr, blue!60!black]   (C)  -- (D);

\draw[arr, orange!70!black] (D.east) to[out=0, in=180] (E1.west);
\draw[arr, orange!70!black] (D.east) to[out=0, in=180] (E2.west);

\draw[arr, green!50!black]  (E1.east) to[out=0, in=180] (F.west);
\draw[arr, green!50!black]  (E2.east) to[out=0, in=180] (F.west);

\draw[arr, green!50!black]  (F) -- (G);

%% ── Phase braces ────────────────────────────────────────────────────
\draw[decorate, decoration={brace, amplitude=5pt, raise=28pt},
      blue!50!black, thick]
    (A.north west) -- (D.north east)
    node[midway, above=36pt, font=\footnotesize\bfseries, blue!60!black]
    {Data Pipeline};

\draw[decorate, decoration={brace, amplitude=5pt, raise=28pt},
      orange!70!black, thick]
    ($(E1.north west)$) -- ($(E1.north east)+(0.0,0)$|-E1.north)
    node[midway, above=36pt, font=\footnotesize\bfseries, orange!70!black]
    {};
%% simpler single label between E1/E2
\node[font=\footnotesize\bfseries, orange!70!black]
    at (11.4, 2.55) {Evaluators};

\draw[decorate, decoration={brace, amplitude=5pt, raise=28pt},
      green!50!black, thick]
    (F.north west) -- (G.north east)
    node[midway, above=36pt, font=\footnotesize\bfseries, green!60!black]
    {Editing};

\end{tikzpicture}%
}
\caption{\textsc{TactileEval} end-to-end pipeline.
\textbf{Data Pipeline} (\textcolor{blue!60!black}{blue}): expert free-text
comments seed a five-category BANA-aligned taxonomy; AMT workers produce 231
structured annotations per family; records are stored as deterministic JSONL splits.
\textbf{Evaluators} (\textcolor{orange!70!black}{orange}): a GPT-4o pilot and a
CLIP feature probe are trained in parallel on the same splits.
\textbf{Editing} (\textcolor{green!60!black}{green}): model diagnoses drive a
few-shot recipe that produces corrected embosser-ready tactile renders.}
\label{fig:pipeline}
\end{figure*}
